Cardinality Constrained Scheduling in Online Models

Makespan minimization on parallel identical machines is a classical and intensively studied problem in scheduling, and a classic example for online algorithm analysis with Graham's famous list scheduling algorithm dating back to the 1960s. In this problem, jobs arrive over a list and upon an arrival, the algorithm needs to assign the job to a machine. The goal is to minimize the makespan, that is, the maximum machine load. In this paper, we consider the variant with an additional cardinality constraint: The algorithm may assign at most $k$ jobs to each machine where $k$ is part of the input. While the offline (strongly NP-hard) variant of cardinality constrained scheduling is well understood and an EPTAS exists here, no non-trivial results are known for the online variant. We fill this gap by making a comprehensive study of various different online models. First, we show that there is a constant competitive algorithm for the problem and further, present a lower bound of $2$ on the competitive ratio of any online algorithm. Motivated by the lower bound, we consider a semi-online variant where upon arrival of a job of size $p$, we are allowed to migrate jobs of total size at most a constant times $p$. This constant is called the migration factor of the algorithm. Algorithms with small migration factors are a common approach to bridge the performance of online algorithms and offline algorithms. One can obtain algorithms with a constant migration factor by rounding the size of each incoming job and then applying an ordinal algorithm to the resulting rounded instance. With this in mind, we also consider the framework of ordinal algorithms and characterize the competitive ratio that can be achieved using the aforementioned approaches.

==> fig/migration_load_pattern_s3toxi-1.tex <==
\begin{figure}[h]
\centering
\begin{tikzpicture}
%basic parameters
\pgfmathsetmacro{\MachW}{0.5}
\pgfmathsetmacro{\MachH}{0.2}
\pgfmathsetmacro{\MachGap}{2.5*\MachW}
\pgfmathsetmacro{\JobH}{0.3}
%\pgfmathsetmacro{\JobLabelShift}{0.1}
\pgfmathsetmacro{\MachLabelShift}{-2.4*\MachH}

%machines
\foreach \a/\b/\c/\d in {	0/0/0/$1$, 
							1/1/0.6*\MachW/$\floor[\big]{\frac{m}{8\kappa}} + 1$,
							2/2/0.6*\MachW/$\floor[\big]{\frac{m}{4\kappa}} + 1$,
							3/2/0/,
							4/3/0.6*\MachW/,
							5/3/0.6*\MachW/$\floor[\big]{\frac{m}{2\kappa}} + 1$,
							6/4/0.6*\MachW/,
							7/4/0.6*\MachW/$\floor[\big]{\frac{m}{\kappa}} + 1$,
							8/5/0/$m$
						}
{
	\draw[thick] 	(\a*\MachW + \b*\MachGap,-\MachH) -- 
					(\a*\MachW + \b*\MachGap,0) -- 
					(\a*\MachW + \b*\MachGap + \MachW,0) node[midway,yshift= \MachLabelShift cm, xshift = \c cm]{\d} -- 
					(\a*\MachW + \b*\MachGap + \MachW,-\MachH);
}
%machine dots
\foreach \a/\b in {1/0,2/1,4/2,6/3,8/4}{
	\draw[thick] (\a*\MachW + \b*\MachGap,0) -- (\a*\MachW + \b*\MachGap + \MachGap,0) node[midway, yshift = -0.7*\MachH cm ] {$\dots$};
}
%jobs
\foreach \a/\b/\aa/\bb/\xs/\xxs/\h/\c/\l in 	
{
	0/0/2/2/0.5/0.5/1/black/$p_1$,
	3/2/8/5/0.5/0.5/1/black/$p_2$,
	5/3/8/5/0.5/0.5/2/mred/$p_2$,
	2/2/2/2/0.5/0.5/3/black/$p_2$,
	3/2/6/4/0.5/0.5/3/black/$p_3$,
	5/3/6/4/0.5/0.5/4/mred/$p_3$,
	2/2/2/2/0.5/0.5/6/black/$p_{\iota^*}$,
	3/2/6/4/0.9/0.9/6/black/$p_{\iota^* + 1}$,
	5/3/6/4/0.9/0.9/7/mred/$p_{\iota^* + 1}$,
	1/1/2/2/0.9/0.3/8/black/$p_{\iota^* + 1}$,
	3/2/4/3/0.9/0.5/8/black/$p_{\iota^* + 2}$,
	2/2/2/2/0.3/0.3/9/black/$p_{\iota^* + 2}$,
	3/2/4/3/0.9/0.5/9/black/$p_{\iota^* + 3}$,
	1/1/2/2/0.5/0.5/11/black/$p_{\tilde{k}}$,
	3/2/4/3/0.8/0.5/11/mred/$p_{\tilde{k}+1}$,
	2/2/2/2/0.3/0.3/12/mred/$p_{\tilde{k}+1}$
}
{
	\draw[color = \c] (\a*\MachW + \xs*\MachW +\b*\MachGap,\h*\JobH) node[rectangle, fill = white, inner sep=0pt, text = \c] {\l} -- (\aa*\MachW + \bb*\MachGap + \xxs*\MachW,\h*\JobH) node[rectangle, fill = white, inner sep=0pt, text = \c] {\l};
}
%job dots
\foreach \a/\b/\h in 
{
	5.5/3.5/5,
	3.5/2.7/10
}
{
	\node at (\a*\MachW + \b*\MachGap,\h*\JobH + 0.3*\JobH) {\vdots};
}
\end{tikzpicture}
\caption{The load pattern in the case $s^*\in\set{3,\dots,\phases-1}$. 
There is some ambiguity marked in red.
Namely, the second row jobs on machines $\floor[\big]{\frac{m}{2\kappa}}+1$ to $m$ are only present if $s^*>3$ and represent multiple placements of jobs of size $p_2$.
If we have $s^* = 3$ the placement pattern is different, and the forth row jobs on $\floor[\big]{\frac{m}{2\kappa}}+1$ to $\floor[\big]{\frac{m}{\kappa}}$ represent two rows.
The sixth row on these machines represents $0$ to $2$ rows depending on $s^*$ and $k$.
Finally, we have $\tilde{k} = k-1$ if $(k-1)\bmod 3 =2$ or both $(k-1)\bmod 3 =1$ and $s^* \bmod 2 = 0$ hold.
Otherwise, $\tilde{k} = k$ and $p_{\tilde{k}+1} = 0$.
%We set $\tilde{k} = k - ((k+1) \bmod 3)$. 
%The last (red) and second to last job (blue) on the machines $\floor{\frac{m}{2}} + 1$ to $m$ are only placed if $\tilde{k} + 1 =k$ or $\tilde{k} + 1= k$, respectively.
} 
\label{fig:pattern1_s=3...xi-1}
\end{figure}
